Older Adults' Preferences for Feedback Cadence from an Exercise Coach Robot

People can respond to feedback and guidance in different ways, and it is important for robots to personalize their interactions and utilize verbal and nonverbal communication cues. We aim to understand how older adults respond to different cadences of verbal and nonverbal feedback of a robot exercise coach. We conducted an online study of older adults, where participants evaluated videos of the robot giving feedback at different cadences for each modality. The results indicate that changing the cadence of one modality affects the perception of both it and the other modality. We can use the results from this study to better design the frequency of the robot coach's feedback during an exercise session with this population.

==> text/05_results.tex <==
We recruited 100 online participants using Prolific, with a criterion of age greater than 60, as we want to focus on older adults' perceptions of the robot. We converted the Likert-style results into numeric values from 1-5 and performed a repeated measures ANOVA with the \textbf{verbal} and \textbf{nonverbal} cadences as the two within-subjects conditions, using the Greenhouse-Geisser corrected p-value. Where we found significance, we then performed a pairwise post-hoc test to determine which pairwise differences between feedback cadence levels are significant. Figure \ref{fig:results} shows the results marked with significant differences.

\subsection{Usefulness}
We did not find any significant effects in the robot's perceived usefulness.

\subsection{Clarity}
We did find a significant difference in the perceived clarity of the robot's \textbf{verbal} feedback ($p<0.05, F(2, 198)=3.26$). Specifically, participants thought the \emph{high} verbal cadence was clearer than the \emph{medium} verbal cadence. 

We also find a significant difference in the perceived clarity of the robot's \textbf{nonverbal} feedback when changing its \textbf{verbal} feedback level ($p<0.01, F(2, 198)=4.39$). The participants saw the \textbf{nonverbal} feedback as less clear when paired with the \emph{low} verbal cadence compared to when paired with the \emph{medium} and \emph{high} verbal cadence. This is what we call a secondary effect, which we will discuss further when evaluating our hypotheses.

\subsection{Timeliness}
There is a significant difference in the perceived timeliness of the robot's \textbf{verbal} feedback when changing its \textbf{nonverbal} feedback level ($p<0.05, F(2, 198)=3.75$), which is also a secondary effect. Participants saw the \textbf{verbal} feedback as more timely with \emph{medium} nonverbal cadence compared to the \emph{low} and \emph{high} levels.

We also find a significant difference in the perceived timeliness of the \textbf{nonverbal} feedback ($p<0.05, F(2, 198)=3.70$). The participants saw the \emph{low} level of nonverbal feedback as less timely than the \emph{medium} level. 

We find a secondary effect with the \textbf{nonverbal} feedback's timeliness; there is a significant difference in the perceived timeliness of the robot's \textbf{nonverbal} feedback when changing its \textbf{verbal} feedback ($p<0.05, F(2, 198)=4.36$). Participants saw the \textbf{nonverbal} feedback as more timely with the \emph{high} verbal level compared to the \emph{low} verbal level.

\subsection{Helpfulness}
We find a significant difference in the perceived helpfulness of the robot's \textbf{verbal} feedback ($p<0.01, F(2,198)=6.47$). Participants saw the \emph{low} level of verbal feedback as less helpful than the \emph{medium} and \emph{high} levels. 

We also find a significant difference in the perceived helpfulness of the robot's \textbf{nonverbal} feedback ($p<0.05, F(2,198)=3.42$). Participants saw the \emph{low} nonverbal level as less helpful than the \emph{medium} level.

% \subsection{Demographics}
% We also examined demographic-related differences in perceptions. Older adults are not a monolith, and we are interested in exploring other factors that could affect the participants' view of the \textbf{verbal} and \textbf{nonverbal} feedback. 

% \paragraph{Gender} We find a significant difference in the perceived usefulness ($p<0.05, F(2, 97)=5.65$) and helpfulness ($p<0.01, F(2, 97)=5.28$) of the robot's \textbf{verbal} feedback between participants of different genders. Those identifying as female rated these measures as higher for the \textbf{verbal} feedback than those identifying as male.

% We also find a significant secondary effect when looking at the differences in perceptions between genders. Participants with different genders viewed the usefulness ($p<0.01, F(2, 97)=5.39$) and helpfulness ($p<0.01, F(2, 97)=5.28$) of the robot's \textbf{verbal} feedback differently when varying its \textbf{nonverbal} frequency. Specifically, those identifying as female rated these measures higher compared to those identifying as male.

% \paragraph{Age} We also grouped participants by age (60s, 70s, 80s, 90s) to determine if there are age-related perception differences within the older adult population. We interestingly find a significant interaction effect between age and the perception of the \textbf{verbal} feedback's usefulness when changing the \textbf{nonverbal} cadence ($p<0.05, F(4, 194)=2.66$). Specifically, when viewing the high \textbf{nonverbal} cadence, participants in their 70s viewed the \textbf{verbal} feedback as more useful compared to those in their 60s.

% We find a significant interaction effect between age and the perception of the \textbf{nonverbal} feedback's clarity ($p<0.05, F(2, 91)=1.49$). When viewing the medium \textbf{nonverbal} cadence, participants in their 60s viewed the \textbf{nonverbal} feedback as less clear than those in their 70s. We also find that when viewing the high \textbf{nonverbal} cadence, participants in their 70s viewed the \textbf{nonverbal} feedback as less clear than those in their 60s or 80s.






